Are Synthetic Corruptions A Reliable Proxy For Real-World Corruptions?

Deep learning (DL) models are widely used in real-world applications but remain vulnerable to distribution shifts, especially due to weather and lighting changes. Collecting diverse real-world data for testing the robustness of DL models is resource-intensive, making synthetic corruptions an attractive alternative for robustness testing. However, are synthetic corruptions a reliable proxy for real-world corruptions? To answer this, we conduct the largest benchmarking study on semantic segmentation models, comparing performance on real-world corruptions and synthetic corruptions datasets. Our results reveal a strong correlation in mean performance, supporting the use of synthetic corruptions for robustness evaluation. We further analyze corruption-specific correlations, providing key insights to understand when synthetic corruptions succeed in representing real-world corruptions. Open-source Code: https://github.com/shashankskagnihotri/benchmarking_robustness/tree/segmentation_david/semantic_segmentation

==> tex_for_figures/correlation_acdc_2dcc.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{plots/2dcc_cityscapes_acdc.pdf}
    \caption{To empirically determine if synthetic common corruptions such that those proposed by \cite{commoncorruptions} truly represent the distribution and domain shifts in the real world we try to find correlations in evaluations on ACDC and 2D Common Corruptions. Each model is trained on the training dataset of the Cityscapes dataset. 
    The y-axis represents values from evaluations on the ACDC dataset, and the x-axis represents values from evaluations on the Common Corruptions at severity=3.
    Starting from the left, we find correlations between ACDC the following: first the mean performance across all common corruptions; second the synthetic brightness corruption; third the synthetic snow corruption; and fourth the synthetic fog corruption. We observe a positive correlation, and strong positive correlation between performance on the ACDC and mean performance against all synthetic common corruption.}
    \label{fig:correlation_2dcc_acdc}
\end{figure*}

==> tex_for_figures/correlation_dataset.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{plots/ade20k_cityscapes.pdf}
    \caption{To find correlations in observations across datasets, here we use the ADE20K dataset and Cityscapes dataset. Each model is trained on the training dataset of the respective dataset on which it is eventually evaluation. 
    The y-axis represents values from evaluations on the ADE20K dataset, and the x-axis represents values from evaluations on the Cityscapes dataset.
    Starting from the left, we find correlations between ADE20K and Cityscapes dataset for have the following: first the i.i.d. performance; second the reliability under $\ell_{\infty}$-norm bounded adversarial attacks; third the reliability under $\ell_{2}$-norm bounded adversarial attacks; and fourth the generalization ability.}
    \label{fig:correlation_ade20k_cityscapes}
\end{figure*}

==> tex_for_figures/teaser.tex <==

%
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
\vspace{-.5cm}
    \centering
    \scalebox{0.94}{
    \begin{tabular}{@{}c@{}c@{}c@{}cc}
    & &
    Input Image & \phantom{a}Ground Truth & \phantom{aa}Prediction \\
    \multirow{2}{*}{\rotatebox{90}{Real World Corruption}} &
    \multirow{2}{*}{\rotatebox{90}{Snow}} &
    \includegraphics[width=0.35\linewidth,valign=t]{workshop_figures/acdc_images_preds/snow_acdc_original_image_(GOPR0604_frame_000413_rgb_anon).png}     
         & 
    \multicolumn{2}{c}{\includegraphics[width=0.7\linewidth,valign=t]{workshop_figures/acdc_images_preds/snow_acdc_predictions_model_mask2former-swinb-cityscapes_(test_GOPR0604_frame_000413_rgb_anon.png_0).png}}
         \\

        &
        \multirow{2}{*}{\rotatebox{90}{Fog}} &
    \includegraphics[width=0.35\linewidth,valign=t]{workshop_figures/acdc_images_preds/fog_acdc_original_image_(GOPR0476_frame_000921_rgb_anon).png}     
         & 
    \multicolumn{2}{c}{\includegraphics[width=0.7\linewidth,valign=t]{workshop_figures/acdc_images_preds/fog_acdc_predictions_model_mask2former-swinb-cityscapes_(test_GOPR0476_frame_000921_rgb_anon.png_0).png}}
         \\

         %%%%%%%%%%%  END REAL WORLD   %%%%%%%%

    \multirow{2}{*}{\rotatebox{90}{Synthetic Corruption}} &
    \multirow{2}{*}{\rotatebox{90}{Snow}} &
    \includegraphics[width=0.35\linewidth,valign=t]{workshop_figures/2dcc_images_preds/snow_input_frankfurt_000000_000294_leftImg8bit.png}     
         & 
    \multicolumn{2}{c}{\includegraphics[width=0.7\linewidth,valign=t]{workshop_figures/2dcc_images_preds/snow_pred_test_frankfurt_000000_000294_leftImg8bit.png_1.png}}
         \\

        &
        \multirow{2}{*}{\rotatebox{90}{Fog}} &
    \includegraphics[width=0.35\linewidth,valign=t]{workshop_figures/2dcc_images_preds/fog_input_frankfurt_000000_000294_leftImg8bit.png}     
         & 
    \multicolumn{2}{c}{\includegraphics[width=0.7\linewidth,valign=t]{workshop_figures/2dcc_images_preds/fog_pred_test_frankfurt_000000_000294_leftImg8bit.png_1.png}}
         \\
    \end{tabular}
    
    }
    \captionof{figure}{Comparing images with weather corruptions captured in the wild (ACDC~\cite{acdc} and images corrupted using synthetic corruptions~\cite{commoncorruptions} and the predictions using a Mask2Former~\cite{cheng2021mask2former} with a Swin-Base~\cite{liu2021Swin} backbone trained on the Cityscapes~\cite{cordts2016cityscapes} dataset.}
    \label{fig:teaser}
\end{center}
}]
